Exploring the Challenges towards Lifelong Fact Learning

So far life-long learning (LLL) has been studied in relatively small-scale and relatively artificial setups. Here, we introduce a new large-scale alternative. What makes the proposed setup more natural and closer to human-like visual systems is threefold: First, we focus on concepts (or facts, as we call them) of varying complexity, ranging from single objects to more complex structures such as objects performing actions, and objects interacting with other objects. Second, as in real-world settings, our setup has a long-tail distribution, an aspect which has mostly been ignored in the LLL context. Third, facts across tasks may share structure (e.g., <person, riding, wave> and <dog, riding, wave>). Facts can also be semantically related (e.g., "liger" relates to seen categories like "tiger" and "lion"). Given the large number of possible facts, a LLL setup seems a natural choice. To avoid model size growing over time and to optimally exploit the semantic relations and structure, we combine it with a visual semantic embedding instead of discrete class labels. We adapt existing datasets with the properties mentioned above into new benchmarks, by dividing them semantically or randomly into disjoint tasks. This leads to two large-scale benchmarks with 906,232 images and 165,150 unique facts, on which we evaluate and analyze state-of-the-art LLL methods.

==> Mid-Scale-Experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}
 \centering
  \caption{\label{tab:fact_4_tasks_random_i2f} Mean average precision for (image to fact) scenario achieved on  each batch at the end of the sequence. Based on clustering the Mid scale dataset 6DS into 4 disjoint groups of facts  }
 \begin{tabular}{ | l | c| c | c | c | c | c |}
 \hline
 Method & $B_1$ &$B_2$&B3 & B4 &all\\  \hline
% %
 Finetuning& 0.466 & 0.264 &0.268&0.831&0.326\\  \hline  	


 Int. Synapses&  0.463 &  0.380 &0.365& 0.746&0.350\\  \hline  

 %{'res_b1': 0.0508878259411037, 'res_b3': 0.088243597590422607, 'res_b2': 0.10210063299330743, 'res_b4': 0.10625575846581828}
 %B2_elastic_reg_1_b1train	0,36	0,3576	0,279	0,462	0,292									
 %Ours on Train& 0.271& 0.246 &0.237&0.377&0.277\\  \hline  
									
 MAS&  &  0.537 &0.446 &0.458& 0.698&0.394\\  \hline  
 %on Traing data only
% %{'res_b1': 0.29504979244916801, 'res_b2': 0.23784487176071828, 'res_b4': 0.39652403591452356, 'res_all': 0.28506532531130085, 'res_b3': 0.23933478694529423}		
 \end{tabular}

\vspace*{-0.2cm} 
 \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{table*}
 \centering
  \caption{\label{tab:fact_4_tasks_disjoint_i2f} Mean average precision achieved on  each batch at the end of the sequence. Based on clustering the Mid scale dataset 6DS into 4 disjoint groups of facts  }
 \begin{tabular}{ | l | c| c | c | c | c | c |}
 \hline
 Method & $B_1$ &$B_2$&B3 & B4 \\  \hline
% %
 Finetuning& 0.0330 & 0.0652  &0.1177&0.1020\\  \hline  	


 Int. Synapses& 0.0598 & 0.0896 &0.0928&0.350\\  \hline  

 %{'res_b1': 0.0508878259411037, 'res_b3': 0.088243597590422607, 'res_b2': 0.10210063299330743, 'res_b4': 0.10625575846581828}
 %B2_elastic_reg_1_b1train	0,36	0,3576	0,279	0,462	0,292									
 %Ours on Train& 0.271& 0.246 &0.237&0.377&0.277\\  \hline  
									
 LwnF& 0.321& 0.16880 &0.229 &0.1058\\  \hline  
% %{'res_b1': 0.29504979244916801, 'res_b2': 0.23784487176071828, 'res_b4': 0.39652403591452356, 'res_all': 0.28506532531130085, 'res_b3': 0.23933478694529423}		
 \end{tabular}

\vspace*{-0.2cm} 
 \end{table*}

==> abstract.tex <==
Lifelong learning (LLL) is a key aspect of the human visual system and seems crucial for truly scalable artificial learning systems operating under real world conditions as well. 
So far, however, lifelong learning in the context of computer vision has been studied mostly in relatively small-scale and relatively artificial setups. Due to the importance of the problem and to speed up progress towards scalable human-like visual systems, we introduce a new benchmark aiming at large scale lifelong learning of a diverse set of semantically structured concepts, denoted as image facts. Facts includes not only single objects, but also more complex structures such as actions, and interactions. They are semantically structured, %and can be extracted by hundreds of thousands from multimodal data
and have a long-tail distribution, posing several new challenges to existing lifelong learning methods.  There are several questions that this paper aims to answer. How do existing life-long learning methods perform on a large number of concepts? What is the effect of  life-long learning losses on recognition accuracy on different concept types (e.g., objects, objects performing actions, and interacting objects/visual relations)? What division of tasks is more helpful to continually learn facts at scale?
How does the long-tail distribution of the facts limit the performance of current methods? In order to address these questions,  we also design a methodology to convert  fact learning datasets to the lifelong learning setup, by dividing it semantically into disjoint tasks and we compared to the case where these tasks are defined randomly. We illustrate this process on a dataset of more than 814.000 images with more than 200,000 facts. We performed extensive experiments with several state-of-the-art LLL methods on the designed  large scale benchmarks. We also comprehensively analyzed the results and discuss interesting findings that are guided by the aforementioned questions. 

==> background.tex <==
In this section we review the LLL methods we evaluate on our benchmark, namely Intelligent Synapses \cite{zenke2017improved} and Memory Aware Synapses \cite{mas}. We also shortly discuss  a Fine-tuning Baseline and an ``upper bound'' by training everything jointly, which violates the lifelong learning scenario.
As argued in the related work section, we adopt the family of LLL approaches that computes the importance of the network parameters for previous tasks and counters catastrophic forgetting by encouraging the important weights of earlier tasks to be preserved during the training of the new task~\cite{kirkpatrick2016overcoming,zenke2017improved,mas}. More concretely, at training step $t$, we have in addition to the new task loss, a regularizer that penalizes changes to the network parameters that are considered important for the previous tasks. In this section, we present the general framework that applies to all of these methods. We denote the loss of training the new Task at time $t$ as $L(\theta)$, where $\theta$ are the parameters of the network such that $\theta_{i}$ is the $i^{th}$  parameter of  an arbitrary  neural network (a deep Neural Network with both convolutional and fully connected layers, in our case). $L(\theta)$ is defined as follows  
\begin{equation}
L(\theta)=L_{n}(\theta)+\frac{\lambda}{2} \omega^{t-1}_{i}(\theta_{i}-\theta^{t-1}_{i})^2
\end{equation}
%$L(\theta)$ is decomposed into two parts   $L_{new}(\theta)$  and a regularizer term defined based on an importance weighting function \Omega_{i}. $L_{new}$ which encourages the network to do well in the facts of the new task.
with $\lambda$ a hyperparameter for the regularizer, $\theta_{i}^{t-1}$ the ``old'' network parameters at time $t-1$, and $\omega_{i}^{t-1}$ a weight indicating the importance of parameter $\theta_i$ for all tasks up to $t-1$. Hence, we tie strong springs on the important parameters at the previous time step (i.e., high $\omega^{t-1}_{i}$) and weak springs on the non-important parameters (i.e., low $\omega^{t-1}_{i}$). This way, we allow changing the latter more freely.  We denote the vector of all the importance weights for all the neurons at time step $t$ as $\mathbf{\omega^{t}}$. After training the first task, the importance weights vector $\mathbf{\omega^{1}}$  is computed to initiate the training process for task 2.  The same process is repeated until we reach the final task. As detailed in the related work, different methods differ in the way this notion  of importance weights is obtained (e.g., ~\cite{kirkpatrick2016overcoming,zenke2017improved,mas}).


\begin{comment}
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.35\textwidth]{figs/sherlock.jpg}
      \caption{The Sherlock modelArchitecture~\cite{elhoseiny2017sherlock}}
      \label{fig1_sherlock}
\end{figure}
\end{comment}
\noindent \textbf{Evaluated LLL Methods and Model } We start by evaluating the $(1)$ Fine-tuning baseline  (i.e., $\omega^{t}=0$)  as a baseline without any life-long Learning loss. This baseline is expected to perform well on the new task, yet suffers from catastrophic forgetting of the knowledge of the old tasks.
Additionally, we compare to two very recent life-long learning approaches: (2) Intelligent Synapses~\cite{zenke2017improved} and (3) {Memory Aware Synapses}~\cite{mas}. In Intelligent Synapses~\cite{zenke2017improved}, $\omega^{t}$ is defined as a per-parameter contribution to the loss.  In contrast {Memory Aware Synapses}, $\omega^{t}$  defines the $\omega^{t}$  based on per-parameter contribution to the final feature activation. Finally, we also include as an upper bound the (4) Joint training, which has a replay access to all the tasks and can go over them for hundreds of epochs. 

In order to study the catastrophic forgetting problem in our life-long learning setup, we choose to use the joint-embedding architecture in~\cite{elhoseiny2017sherlock} as the backbone architecture on which we incorporate the above losses and compare their performance. Fig~\ref{fig1_sherlock} shows the Sherlock model architecture. For details we refer to~\cite{elhoseiny2017sherlock}. %adapted to life-long learning setup.  


%\subsection
\noindent{\bf Adapting LLL methods to Fact learning}
The main difference between models for fact learning and the models for image classification used in standard LLL setups, is in the output layer. Instead of a softmax output, the last layer consists of a projection onto an embedding space. 
As discussed in the related work section, this is problematic for some of the LLL methods, such as~\cite{lee2017overcoming}, that assume a different output space for each task. 
For model-based approaches, as the one selected above, this does not form a problem.  

The major difference in setup caused by the switch to a fact learning LLL setup, lies in the fact that now the full model is shared. This makes the problem significantly more challenging and could cause even more catastrophic forgetting. On the other hand, facts from different tasks can have some overlap -- even a distance equal to zero, if one fact is a subset of the other. While this favors knowledge transfer between tasks in general and opens up opportunities for improved continual learning, it is unclear what the effect of this will be for the existing LLL algorithms, which have not been designed for such a setting. 

\noindent{\bf Evaluation metrics}
\cite{elhoseiny2017sherlock} have proposed two different evaluation criteria to be used with their dataset. Both are based on a retrieval setup, either retrieving facts given images (i2f), based on the top 1, top 5, or top 10 accuracy, or retrieving images given facts (f2i), based on mean average precision (MAP). Given the long tail distribution of the large scale dataset, computing mean average precision does, however, not make much sense.  
\tinne{improve discussion why MAP is not good with long-tail as in large scale dataset}
%We study three methods that  defines $\omega{t}$ differently. The first baseline is Fine-tuning which means no life-long learning code (i.e., $\omega{t}=0$).    
%Fine-tuning trains {Joint Training} 





%a change in the parameters $\theta(t) = [\theta_k(t)]$ by an infinitesimal amount $\delta(t) = [\delta_k(t)]$ results in a change in the loss $L(\theta)$ approximated by:
%\begin{equation}
%L(\theta(t) + \delta(t)) -L(\theta(t))\approx \sum_k g_k(t)\delta_k(t)
%\end{equation}
%with $g_k(t) = \frac{\partial{L}}{\partial{\theta_k}}$ the gradient of the loss with respect to parameter $\theta_k$.
%Based on this, the 
%total change in the loss from the point when the learning started up to convergence for a given task 
%change in the loss over one step in the training procedure can be decomposed in contributions $\omega_k^\mu$ from each of the parameters $\theta_k$: 
%summing over the infinitesimal changes
%\begin{equation}
% \int_{t^{\mu-1}}^{t^\mu}g(\theta(t))\theta'(t)dt  =  \sum_k \underbrace{\int_{t^{\mu-1}}^{t^\mu} g_k(\theta(t)) \theta^{'}_k(t) dt}_{= - \omega_k^\mu} \\
% & \triangleq & - \sum_k{\omega_k^\mu}
%\end{equation}
%The contribution of one particular parameter $\theta_k$ to the total change in the loss, from the point when the learning started up to convergence for a given task, $L(\theta_1) - L(\theta_0)$, can then be obtained by summing its contributions $\omega_k^\mu$ along the training trajectory.
%\int_{t^{u-1}}^{t^u} g(\theta(t))theta^'(t)dt=\sum_k\int_{t^{u-1}}^{t^u}  
%As such they  update an importance value of each parameter $\theta_k$ with respect to the task being learned.


%This procedure allows to compute the importance of the parameters in an online fashion. However, it is based on the dynamics of the learning process and suffers from the drawbacks mentioned earlier in the related work (section~\ref{sec:related_work}). What we actually need is an online method for computing and adapting  the importance of the parameters while the network is actively tested on new input data.


% TT: Leave out ? We do not really use this, do we ?
% Also keep in mind that if a set of datapoints is quite important to preserve, it can be combined with a larger multiplier in the overall importance of the parameters.
%RA: Yes we can leave it out

% TT: unclear whether in text below this L2-norm is to be used instead of L_new or instead of the regularizer, or instead of the function F
%RA:it is instead of the function F
%where all the network parameters are shared, 


==> large_scale_experiments.tex <==

For the large scale sequence of tasks, as described in section~\ref{sec:benchmark},  we compare the methods described in Sec~\ref{sec:methods}. Tables~\ref{tab:arge_scale_semantic} and ~\ref{tab:large_scale_random} shows the performance on the evaluated methods on both the semantic and the random splits.  In contrast to the mid-scale dataset, the LLL methods improvement over fine-tuning is relatively less significant due to the effect of the long-tail distribution  and the large concept space ( not present in the mid-scale dataset). However, MAS~\cite{mas} and ExpertGate~\cite{aljundi2016expert} performs the best among the evaluated methods. We argue that the reason why MAS is performing the best is due to its capability to adapt on unseen data and since the importance is computed based on sensitivity in the output space. This is critical to perform well in this joint-embedding task.
ExpertGate~\cite{aljundi2016expert} has shown the strongest performance among all the methods and is the closest to the joint training upper bound. However, note that ExpertGate requires storing the models of all the tasks(i.e., $8$ times bigger memory complexity compared to the remaining methods). \mohamed{revise after we get the new IMM models with new regualarizer } Also, note that Incremental Moment Matching (IMM) does not perform well in both random and the semantic. We argue that the reason is that averaging the models significantly disturb the output space which is key for good performance in this benchmark.  



\textbf{Semantic vs Random Split.}
Also note that Finetuning in the semantic-split gradually increase from the first to the last task clearly indicating the catastrophic forgetting problem.   This effect is less severe in the random split for fine-tuning due to the similarity between the tasks.  Contrasting  tables~\ref{tab:arge_scale_semantic} and ~\ref{tab:large_scale_random}, we can clearly see a better performance on most methods on the random split vs the semantic split. 

\textbf{Generalized LLL Performance.} 





%The LLL method, on the other hand, yields significantly more balanced results over all batches/tasks: it effectively fights the forgetting, within certain limits, and distributes the errors more fairly over all tasks. While it improves over the Finetuning baseline on average, it is still clearly below the results obtained by joint learning.





  \begin{table}
\centering
\scalebox{0.45}
{
\begin{tabular}{@{}|l|r|r|r|r|r|r|r|r|r|r|@{}} \hline 
 & {\boldmath\textbf{Fine-tune}} & {\boldmath\textbf{Int.Synapses}} & {\boldmath\textbf{ExpGate}} & {\boldmath\textbf{MAS}} & {\boldmath\textbf{IMM (mean)}} & {\boldmath\textbf{IMM l2 
(mean)}} & {\boldmath\textbf{IMM l2 (mode)}}& {\boldmath\textbf{IMM l2 (mode, $\lambda=0.01$)}} &{\boldmath\textbf{IMM l2 (mode, $\lambda=0.1$)}} & {\boldmath\textbf{Joint}}\\ \hline
\boldmath\textbf{T1} & 9.97 & 11.75 & 12.2 & 14.21 & 3.34 & 5.54 &5.64 &  14.55 &  12.19 & 21.34\\ \hline
\boldmath\textbf{T2} & 12.09 & 12.89 & 12.94 & 13.62 & 5.26 & 17.25 & 3.95  & 11.07 &   7.19 & 8.18\\ \hline
\boldmath\textbf{T3} & 9.62 & 12.34 & 32.84 & 12.18 & 9.38 & 5.89 & 6.38 &  14.07  &  7.05& 36.49\\ \hline
\boldmath\textbf{T4} & 25.24 & 28.44 & 39.11 & 29.39 & 31.33 & 22.43 & 2.39 &  33.35 &   30.33 & 41.79\\ \hline
\boldmath\textbf{T5} & 15.6 & 16.17 & 16.98 & 17.1 & 4.42 & 8.44 & 2.21&   13.92&   10.44& 29.22\\ \hline
\boldmath\textbf{T6} & 22.73 & 26.97 & 32.57 & 29.72 & 3.45 & 13.02 &2.56&   50.18  & 41.30 &30.17\\ \hline
\boldmath\textbf{T7} & 21.92 & 22.89 & 20.37 & 23.29 & 12.04 & 18.76 & 2.44&   21.56&  16.86&17.2\\ \hline
\boldmath\textbf{T8} & 39.33 & 31.77 & 14.4 & 31.88 & 8.31 & 15.39 & 7.33 &   14.82 &   12.83 &15.81\\ \hline
\boldmath\textbf{average} & \boldmath\textbf{19.56} & \boldmath\textbf{20.40} & \boldmath\textbf{22.67} & \boldmath\textbf{21.42} & \boldmath\textbf{9.69} & \boldmath\textbf{13.34} & \textbf{4.11}&  \textbf{ 21.69}&   \textbf{17.27}& \boldmath\textbf{25.025}\\ \hline
\boldmath\textbf{generalized} & \boldmath\textbf{2.13} & \boldmath\textbf{2.36} & \boldmath\textbf{xxx} & \boldmath\textbf{2.67} & \boldmath\textbf{xxx} & \boldmath\textbf{xxx} & \boldmath\textbf{xxx}\\ \hline
\end{tabular}
}
\label{tab:large_scale_semantic}
\caption{Top5 Acc: Large Scale Experiment (Semantic Split)\rahaf{check the repeated rows values}}
\end{table}

 
  \begin{table}
\centering
\scalebox{0.5}
{
\begin{tabular}{@{}|l|r|r|r|r|r|r|r|@{}} \hline
 & {\boldmath\textbf{Fine-tune}} & {\boldmath\textbf{Int.Synapses}} & {\boldmath\textbf{MAS}} & {\boldmath\textbf{IMM}} & {\boldmath\textbf{IMM l2(mean)}} & {\boldmath\textbf{IMM l2(mode)}} &  {\boldmath\textbf{IMM l2(mode, $\lambda=0.01$)}}\\ \hline
\boldmath\textbf{T1} & 12.09 & 14.38 & 15.59 & 3.67 & 5.08 5.10 &   18.51\\
\boldmath\textbf{T2} & 19.32 & 20.64 & 24.86 & 6.51 & 3.61 & 7.93  & 24.30\\
\boldmath\textbf{T3} & 19.95 & 24.28 & 27.45 & 9.74 & 5.96& 4.47 &   26.13\\
\boldmath\textbf{T4} & 15.11 & 19.21 & 22.53 & 0.55 & 2.18 & 28.32 &  22.36\\
\boldmath\textbf{T5} & 15.24 & 19.68 & 22.26 & 0.37 & 1.73 & 4.67 &   23.91\\
\boldmath\textbf{T6} & 11.6 & 14.84 & 16.15 & 0.53 & 2.62 & 30.11 &   16.76\\
\boldmath\textbf{T7} & 19.31 & 20.99 & 22.36 & 1.88 & 1.51 & 30.11 &   16.76\\
\boldmath\textbf{T8} & 45.9 & 36.56 & 35.57 & 7.97 & 8.18 & 10.21&   20.80\\
\boldmath\textbf{average} & \boldmath\textbf{19.81} & \boldmath\textbf{21.32} & \boldmath\textbf{23.346} & \boldmath\textbf{3.90} & \boldmath\textbf{3.85}\\ \hline 
\boldmath\textbf{generalized} & \boldmath\textbf{} & \boldmath\textbf{} & \boldmath\textbf{} & \boldmath\textbf{} & \boldmath\textbf{}\\ \hline 
\end{tabular}
}
\label{tab:large_scale_random}
\caption{Top 5 Acc: Large Scale Experiment (Random  Split) \rahaf{check the repeated rows values}}
\end{table}

 
In Figure~\ref{fig:taskperform}, we show the performance for each task, for the different methods, as a function of the number of training images for the facts in the x-Axis. Looking at the figure, from top-left to right bottom, we can observe the natural increase of the fine-tuning overall performance. Life-long learning methods like Int.Synapses are more balanced yet still competitive to finetuning. It is interesting to us to see the behavior of Int.Synapses with the tail, and how big is its gap with fine-tuning at earlier tasks. We note that MAS performs overall similar to the Int.Synapses approach, slightly better than FineTuning, but worse than Joint training (where joint training does not follow the LLL constraint). Further more,  it interesting to see that sometimes Int.Synapses performs better that Joint Training in facts with earlier tasks (e.g., Task2). Joint training seems to outperform especially on ‘easier’ tasks (where mean for joint is higher), as it specializes less. More  detailed analysis and interpretation is attached  in the supplemental about the long-tail behavior and the types of facts in each Task.
 
\begin{figure*}
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1}
\center
 \begin{tabular}{cccc}
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T1untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T2untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T3untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T4untill_T8_semantic.png}\\
\includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T5untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T6untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T7untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T8untill_T8_semantic.png}\\
\end{tabular}
\caption{(New Semantic Split)Large Scale Experiment: Performance in low-shot scenario for each task after training all tasks for Joint, Int.Synapses, Finetune.
For each task, we group facts based on how frequently they occur (x-axis) and show how the top 5 performance varies as a function thereof.}
\label{fig:taskperform}
\end{figure*}
\begin{comment}
\begin{figure*}
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1}
\center
 \begin{tabular}{cccc}
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T1untill_T8_random.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T2untill_T8_random.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T3untill_T8_random.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T4untill_T8_random.png}\\
\includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T5untill_T8_random.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T6untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T7untill_T8_semantic.png}&
 \includegraphics[height=0.2\textwidth,width=0.25\textwidth]{figs/T8untill_T8_semantic.png}\\
\end{tabular}
\caption{(New Random Split) Large Scale Experiment: Performance in low-shot scenario for each task after training all tasks for Joint, Int.Synapses, Finetune.
For each task, we group facts based on how frequently they occur (x-axis) and show how the top 5 performance varies as a function thereof.}
\label{fig:taskperform}

\end{figure*}
\end{comment}

 \begin{comment}
\begin{figure*}
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{1}
\center
 \begin{tabular}{cccc}
 \includegraphics[width=0.25\textwidth]{T1_K5}&
 \includegraphics[width=0.25\textwidth]{T2_K5}&
 \includegraphics[width=0.25\textwidth]{T3_K5}&
 \includegraphics[width=0.25\textwidth]{T4_K5}\\
\includegraphics[width=0.25\textwidth]{T5_K5}&
 \includegraphics[width=0.25\textwidth]{T6_K5}&
 \includegraphics[width=0.25\textwidth]{T7_K5}&
 \includegraphics[width=0.25\textwidth]{T8_K5}\\
\end{tabular}
\caption{Large Scale Experiment: Performance in low-shot scenario for each task after training all tasks for Joint, Int.Synapses, Finetune.
For each task, we group facts based on how frequently they occur (x-axis) and show how the top 5 performance varies as a function thereof.}
\label{fig:taskperform}
\end{figure*}
 \end{comment}



\begin{comment}
  \begin{table*}[h!]
 %\small
%\setlength{\tabcolsep}{4pt}
%\renewcommand{\arraystretch}{1.2}
\centering
\scriptsize
 {
 \begin{tabular}{|  l | rrrr | rrrr | rrrr |}
 \hline
&\multicolumn{4}{c|}{Top 1}&\multicolumn{4}{c|}{Top 5}&\multicolumn{4}{c|}{Top 10}\\
&FineTune&Int.Synapses&{MAS}&Joint&FineTune&Int.Synapses&{MAS}&Joint&FineTune&Int.Synapses&{MAS}&Joint\\\hline
T1&5.96&6.08&6.4&11.55&9.97&11.75& 12.97&21.34&14.12&16.20& 17.2&26.39\\
{T2}&9.92&10.98&10.23&6.69&12.09&12.89&12.17 &8.18&13.93&14.51&13.75 &9.61\\
T3&8.37&10.87&9.96&33.11&9.62&12.34&9.96 &36.49&11.17&13.99&13.17 &39.34\\
T4&24.05&26.94&23.90&38.47&25.24&28.44&25.04 &41.79&26.40&30.16&26.42 &44.51\\
{T5}&14.26&15.06&15.43&27.21&15.60&16.17&16.44 &29.22&16.84&16.83&16.44 &30.75\\
T6&13.42&15.28&16.46&15.77&22.73&26.97& 31.01&30.17&27.78&36.01& 39.14&39.75\\
T7&19.30&19.89&20.32&15.01&21.92&22.89& 24.01&17.20&23.82&25.31&26.13 &19.06\\
T8&33.86&27.26& 27.11 &12.66&39.33&31.77& 31.69&15.81&41.64&34.18& 33.93 &18.42\\\hline
average&16.14&16.55&16.23&20.06&19.56&20.40& 20.6&25.02&21.96&23.40& 23.46& 28.48\\\hline
\end{tabular}
 \caption{Large Scale Experiment: Top1, Top5, Top10.}
 \label{table_lsc}
 }
 \end{table*}
\end{comment}
 






%\end{itemize}


% every model has been trained on each of the four tasks consecutively for 300 epochs. 




%When looking at what our method does when activating the adaptation of the weight importance on the test phased between the different steps, we can notice the fairness among all the subsets and see how the methods does quite a good jobs in fighting the forgetting. 

 
% \subsection{Large scale sequence analysis}
 
%As illustrated earlier, joint training is an upper point We find it interesting to see  sometimes life-long learning methods behaves better and hence means. 

%Clearly, performance improves significantly when focusing on the more frequent facts. 
 
 
%\subsection{}
%To better understand our large scale part of the benchmark, in Table \ref{table_lsc} we additionally show the results of the second lifelong learning (LLL) approach, MAS, which is introduced in \cite{mas} and we already evaluated on the mid-scale 6DS dataset in the main paper.


%\textbf{{\color{blue}Highlight:} MAS added to table4 for LSC dataset, shown in bold}

\subsection{Effect of Life-long Learning loss On different Fact types}
\label{ss_effect}
 
 Fig~\ref{fig:lll_reg_effect} shows that how the additional cost of existing long learning methods affect the learning of the new task based on complexity. The drop of the performance of the  Task8 (last task) for S facts (objects like <dog>, <cat>) is minimal since fine-tuning is 96.5\% and MAS is 95.4\% (within 1\%). Going to more complex SP facts like (e.g., \fact{dog, jumping}), the performance gap increases to more than 9\% on Task 8 (31.0\% fine-tuning,   23.0\% MAS, and 22.6\% Int.Synapses). The LLL regularization becomes even more severe on the SPO facts (e.g. <person, riding, horse>) reaching  ~15\% (50.8\% fine-tuning,   37.1\% MAS, and 35.6\% Int.Synapses). It is worth mentioning that, the MAS behaves relatively better than Int.Synapses as the fact complexity increases. 
 \begin{figure}[h!]
\centering
 \includegraphics[width=0.32\textwidth,height=0.25\textwidth]{figs/T8_untill_T8_S.jpg} \includegraphics[width=0.32\textwidth,height=0.25\textwidth]{figs/T8_untill_T8_SP.jpg} \includegraphics[width=0.32\textwidth,height=0.25\textwidth]{figs/T8_untill_T8_SPO.jpg}
\caption{Life-long Learning Regularization effect becomes more severe as tasks goes more complex}
\label{fig:lll_reg_effect}
\end{figure}

 
%\subsection{Overall Performance}
% Figure~\ref{fig:overall} shows  the Top5 Performance for all the test images.  The prediction of each image  in this figure is not restricted  to belong to facts of a particular Task (i.e., the union of all facts are possible facts including unseen facts). This figure shows an overview of fact level understanding at the end of training. 
 
%\begin{figure}[h!]
%\centering
% \includegraphics[width=0.7\textwidth]{overall}
%\caption{Cross Task Top5  Performance including test images of facts not seen by any of the Tasks:  the performance of the union of the test sets and the prediction of each image is not restricted to belong to facts of a particular Task (i.e., the union of all facts are possible predictions).}
%\label{fig:overall}
%\end{figure}

\textbf{Behavior on the Head and Tail  Facts:} . It turns out that Fine-tuning actually works better on facts with a small number of examples (the tail), while life-long learning methods like MAS~\cite{mas} or Int. Synapses~\cite{poole2017intelligent} work better on the head. This is due to two reasons. First, the LLL regularization affects the tail classes which are more likely to be SP and SPO facts as we illustrate earlier in Sec~\ref{ss_effect}. Second,  the low-shot facts contribute very little to the importance weights assigned by either MAS or Int. Synapses, where every example is equally contributing to the importance. Hence, the low-shot facts are at a disadvantage. This shows the bias of existing LLL method against the Tail. We show that the behavior of existing LLL techniques changes significantly on the tail (facts with little training images). Simple LLL baselines perform better, while the behavior of frequent facts is consistent with the literature. 

\begin{figure}[ht!]
\centering
 %\includegraphics[width=0.8\textwidth]{overall_till50}
  \includegraphics[width=0.7\textwidth]{figs/Fig_overall_few}
\caption{Zoomed in Version of Fig.~\ref{fig:overall} for facts that have less than 50 training images. This shows that Fine-tuning has an edge for facts that belong to the tail (low-number of training examples). This motivates the next analysis that we did for the set of Facts that have less than 5 training examples (shown in the following tables)}
\label{fig:zoom}
\end{figure}


\subsection{Detailed Analysis}


%Now we discuss how every task starts to suffer from forgetting moving forward from Task 1. Fig.~\ref{fig_forgetting_eachmodel} shows an interpretation on the behavior of these curves based on the correlation between the Tasks.%It is interesting to see how T5 benefits all the tasks. This could be connected by the nature of Tasks in T5 (6321 objects (S) , 24381 object with actions (SP), and 42364 interactions SPOs); see Table~\ref{tbl_lsc_stats}. Also the overlap shown in the statistic we presented in this supplementary in Tables~\ref{tbl_lsc_overlap_sbj} and ~\ref{tbl_lsc_overlap_prd} }



 Figure ~\ref{fig_forgetting_eachmodel} shows the forgetting over the learning sequence for the three methods analyzed : Finetuning, Intelligent Synapses and Memory Aware Synapses. Each model has been evaluated throughout the entire learning sequence (from Task 1 to Task 8) on the data (B) of the task at hand and on data of every previous tasks. Plots in different colors show how much of the initially learned concepts keep being correctly classified after each new learned task. All curves initially plunge, but most of them recovers moving further in the sequence. For example, after tasks 5, all previous encountered data are recognize better.This unique behavior can be seen as part of the characteristic of the our proposed benchmark. Using triplets S,P,O instead of class labels implies more sharing among different tasks and the relatedness among clusters can be helpful in learning a long task sequence. To further comment on these conclusion, we propose  Figure ~\ref{fig_forgetting_eachmodel_2}. Here, we inspect the level of relatedness among clusters using as reference a model trained only on one Task at the time. Evaluating this model on all possible sets of data (B from 1 to 8), one can assess how close are the training data and the data from a different task. If a model trained on data of task $i$ performs somewhat correctly on task $j$ then it can be concluded a relatedness between data of task $i$ and $j$ .It is worthwhile noticing that relatedness and forgetting trends are similar, but life long learning methods still perform better than disjoint training for each task individually Tables $9$, $10$, $11$, $12$.
 
 
 %~\ref{relatedness}, ~\ref{forgetting_finetuning} ,~\ref{forgetting_syn}, ~\ref{forgetting_mas} 
 % The Heatmap and the dashed lines of figure ~\ref{fig_forgetting_eachmodel_2} depicts how some clusters    



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Forgetting in a GRID
\begin{figure*}[h!]
\begin{center}
\includegraphics[width=1.0\textwidth]{figs/Finetuning_Forgetting.png}
\includegraphics[width=1.0\textwidth]{figs/Int_Synapses_Forgetting.png}
\includegraphics[width=1.0\textwidth]{figs/MAS_Forgetting.png}
\end{center}
\caption{Forgetting along the learning sequence for the three analyzed methods: Finetuning, Intelligent Synapses and Memory Aware Synapses.}
\label{fig_forgetting_eachmodel}
\end{figure*}

\begin{figure*}[h!]
\begin{center}
\includegraphics[width=0.4\textwidth]{figs/Sharing_among_tasks_plot.png}
\includegraphics[width=0.4\textwidth]{figs/Sharing_among_tasks.png}
\end{center}
\caption{The dashed linegraph shows the performance of model trained on task $i$ and evaluated over data of all previous tasks of the sequence  $j<i$. The Heatmap indicates the performance of a model trained on Task $i$ data only but tested on all possible Tasks $j$.}
\label{fig_forgetting_eachmodel_2}
\end{figure*}


\subsection{}



\section{compositional generalization}
\textbf{add also per task vs all}
We analyzed \emph{compositional} \emph{generalization} performance of tail facts.  We also the behavior of every task \emph{from head to tail}. 



==> mid_scale_experiments.tex <==
\begin{table}
\centering
\scalebox{0.7}
{
\begin{tabular}{@{}lrrrrrrrrrrrrrr@{}} \toprule
\boldmath\textbf{Random Split} &  & \multicolumn{1}{l}{standard} &  &  &  &  &  & \multicolumn{1}{l}{generalized} &  &  &  &  & \multicolumn{1}{l}{Drop (standard to generalized )} & \\ \midrule
 & \multicolumn{1}{l}{T1} & \multicolumn{1}{l}{T2} & \multicolumn{1}{l}{T3} & \multicolumn{1}{l}{T4} & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{mean per example} & \multicolumn{1}{l}{T1} & \multicolumn{1}{l}{T2} & \multicolumn{1}{l}{T3} & \multicolumn{1}{l}{T4} & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{mean per example} & \multicolumn{1}{l}{Drop (standard-generalized per task(} & \multicolumn{1}{l}{Drop (standard-generalized per example)}\\
\boldmath\textbf{ExpertGate} & 82.46 & 59.28 & 62.92 & 58.75 & 65.85 & 65.56 & 49.31 & 48.79 & 41.59 & 48.56 & 47.06 & 47.01 & 18.79 & 18.55\\
\boldmath\textbf{FineTune} & 82.01 & 46.3 & 52.44 & 88.32 & 67.27 & 67.47 & 42.65 & 34.68 & 22.66 & 83.44 & 45.86 & 46.42 & 21.41 & 21.05\\
\boldmath\textbf{IMM(0.1)} & 91.85 & 63.43 & 75.73 & 70.48 & 75.37 & 75.17 & 75.92 & 53.18 & 55.65 & 57.14 & 60.47 & 60.25 & 14.9 & 14.92\\
\boldmath\textbf{IMM(0.01)} & 88.09 & 75.24 & 83.66 & 69.27 & 79.06 & 78.85 & 61.18 & 64.48 & 70.73 & 51.34 & 61.93 & 61.81 & 17.13 & 17.04\\
\boldmath\textbf{MAS} & 89.62 & 70.98 & 75.87 & 85.06 & 80.38 & 80.38 & 55.27 & 52.72 & 54.58 & 78.02 & 60.15 & 60.5 & 20.23 & 19.87\\
\boldmath\textbf{Syn Int} & 85.08 & 65.31 & 68.64 & 87.03 & 76.51 & 76.6 & 49.01 & 43.95 & 42.89 & 81.58 & 54.36 & 54.85 & 22.16 & 21.75\\
\boldmath\textbf{Joint} & 91.22 & 78.41 & 87.82 & 75.97 & 83.35 & 83.2 & 72.89 & 69.8 & 81.46 & 68.86 & 73.25 & 73.26 & 10.1 & 9.94\\ \bottomrule
\end{tabular}
}
\caption{Random Split (Mid-scale} 
\label{tab:midscale_random}
\end{table}

\begin{table}
\centering
\begin{tabular}{lrrrrrrrrrrrrrr}
\boldmath\textbf{Semantic Split} &  & \multicolumn{1}{l}{standard} &  &  &  &  &  & \multicolumn{1}{l}{generalized} &  &  &  &  & \multicolumn{1}{l}{Drop (standard to generalized )} & \\
 & \multicolumn{1}{l}{T1} & \multicolumn{1}{l}{T2} & \multicolumn{1}{l}{T3} & \multicolumn{1}{l}{T4} & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{mean per example} & \multicolumn{1}{l}{T1} & \multicolumn{1}{l}{T2} & \multicolumn{1}{l}{T3} & \multicolumn{1}{l}{T4} & \multicolumn{1}{l}{mean} & \multicolumn{1}{l}{mean per example} & \multicolumn{1}{l}{per task} & \multicolumn{1}{l}{per example}\\
\boldmath\textbf{ExpertGate} & 65.95 & 64.69 & 59.4 & 12.5 & 50.64 & 62.15 & 58.81 & 79.86 & 49.61 & 9.49 & 49.44 & 57.16 & 1.19 & 4.99\\
\boldmath\textbf{FineTune} & 22.97 & 35.11 & 31.71 & 15.19 & 26.25 & 25.64 & 10.41 & 33.61 & 0 & 15.19 & 14.8 & 11.2 & 11.44 & 14.44\\
\boldmath\textbf{IMM(0.1)} & 59.09 & 90.35 & 60.29 & 11.08 & 55.2 & 60.62 & 34.74 & 63.45 & 58.09 & 0.79 & 39.27 & 40.87 & 15.93 & 19.75\\
\boldmath\textbf{IMM(0.01)} & 65.74 & 91.32 & 63.27 & 12.82 & 58.29 & 65.72 & 40.39 & 60.62 & 43.28 & 8.7 & 38.25 & 41.76 & 20.04 & 23.96\\
\boldmath\textbf{MAS} & 32.46 & 47.27 & 34.8 & 12.97 & 31.87 & 33.67 & 11.74 & 37.17 & 0 & 12.97 & 15.47 & 12.37 & 16.4 & 21.3\\
\boldmath\textbf{Syn Int} & 23.21 & 35.18 & 32.01 & 8.54 & 24.73 & 25.56 & 10.44 & 33.72 & 0 & 8.54 & 13.18 & 10.94 & 11.56 & 14.62\\
\boldmath\textbf{Joint} & 81.22 & 57.04 & 81.47 & 21.2 & 60.23 & 75.88 & 73.58 & 77.04 & 72.75 & 61.55 & 71.23 & 73.26 & -11 & 2.62\end{tabular}
\caption{Mid Scale Experiment (Semantic Split)\rahaf{TODO:check the random performance on T4. check the performance before t4. Can you check why T2 performance of IMM is too high and much higher than joint training? }} 
\label{tab:midscale_semantic}
\end{table}



%We start our study with a mid scale dataset, where we aim to understand the difference in behavior of the LLL methods and baselines, regarding the relatedness degree between the tasks that are learned in a sequence. Then we move on to the large scale setup.
% \tinne{Do we have numbers for the joint training on the mid scale dataset ?}
%Rahaf Already added
Tables~\ref{tab:fact_4_tasks_random_i2f} and ~\ref{tab:fact_4_tasks_disjoint_i2f} shows the Top1 accuracy performance for the random and the semantic split. 
%\tinne{Probably way too long; just trying to say something meaningful about these numbers}
If we compare the two tables, it is clear that the numbers for the setting with disjoint groups are significantly lower than those for the random splits. With random splits, there is still a bigger overlap between facts. Given that the Sherlock model~\cite{elhoseiny2017sherlock} has separate branches for $S$ vs. $P$ and $O$, a fair amount of training data for later tasks may still be relevant for the older tasks, reducing the amount of catastrophic forgetting.  Numbers for the disjoint groups obtained by clustering, on the other hand, show it's a much more difficult task. %Indeed, this is the most challenging situation that can be faced by a continual learning agent. 
%\rahaf {I am not convinced about this sentence}
%\tinne{Agree: joint training is also much lower for B4. Commented this out.}
Focusing on the results obtained with FineTuning, we observe catastrophic forgetting of the older tasks, for both settings, but especially for the case of disjoint groups. 
%also the performance on the new task is much lower. While this may accidentally be a more difficult batch than B4 for the random splits, it could also explained by a reduced amount of forward knowledge transfer, given the more disjoint nature of tasks. 
%\rahaf{Is there a long tail in the mid dataset?}
Comparing the LLL methods with the Finetuning baseline, we see that, in spite of the overlap between facts that's not explicitly modeled, they still manage to save a reasonable amount of the previous groups of facts knowledge and improve the overall numbers, in both settings.
Overall, the numbers achieved by the sequentially trained models are considerably lower than joint training, especially in the disjoint groups of facts. Joint Training has the advantage of visiting all the data as many times as it needs to learn something meaningful.

Finally the results that the generalized LLL performance gets significantly lower compared to the average per task performance. 
%  \begin{table}
%  \footnotesize
%  \centering
%   \caption{\label{tab:fact_4_tasks_random_i2f} Top 5 Accuracy  (image to fact) scenario achieved on  each task at the end of the sequence. Based on splitting the Mid scale dataset 6DS into 4 random sets of facts. * assumes access to all the data in one learning phase  }
%  \begin{tabular}{ | l | c| c | c | c | c | c |c|}
%  \hline
%  Method & $T_1$ &$T_2$&$T_3$ & $T_4$ &avg& generalized \\  \hline
% % %
%  Finetuning& 46.6 & 26.4 &26.8&83.1&45.7 &32.7\\  \hline  
% IS~\cite{zenke2017improved}& 46.3 &  38.0 &36.5& 74.6&48.8 &35.08 \\  \hline  		
%  MAS~\cite{mas} &  53.7 &44.6 &45.8& 69.8&53.4 &39.4\\  \hline  
%  Joint Training*&75.4&63.7& 79.3&56.9&68.8 & 58.9\\ \hline
%  %on Traing data only
% % %{'res_b1': 0.29504979244916801, 'res_b2': 0.23784487176071828, 'res_b4': 0.39652403591452356, 'res_all': 0.28506532531130085, 'res_b3': 0.23933478694529423}		
%  \end{tabular}
%  \vspace*{-0.2cm} 
%  \end{table}
 
\begin{table}
\footnotesize
 \centering
  \caption{\label{tab:fact_4_tasks_random_i2f} (NEW RERSULTS) Top 5 Accuracy  (image to fact) scenario achieved on  each task at the end of the sequence. Based on splitting the Mid scale dataset 6DS into 4 semantic sets of facts. * assumes access to all the data in one learning phase  }
 \begin{tabular}{ | l | c| c | c | c | c | c |c|}
 \hline
 Method & $T_1$ &$T_2$&$T_3$ & $T_4$ &avg& generalized \\  \hline
% %
 Finetuning& 22.97 & 35.11 &31.70&15.19&  & \\  \hline  
IS~\cite{zenke2017improved}& 23.21&   35.17 &32.01& 8.54& & \\  \hline  		
 MAS~\cite{mas} &  32.45 &47.27 &34.80& 12.97& &\\  \hline  
 Joint Training*&75.4&63.7& 79.3&56.9& & \\ \hline
 %on Traing data only
% %{'res_b1': 0.29504979244916801, 'res_b2': 0.23784487176071828, 'res_b4': 0.39652403591452356, 'res_all': 0.28506532531130085, 'res_b3': 0.23933478694529423}		
 \end{tabular}
 
 
 
 


\vspace*{-0.2cm} 
 \end{table}

 \begin{table}
 \footnotesize
 \centering
  \caption{\label{tab:fact_4_tasks_disjoint_i2f}  Top 5 Accuracy  achieved on  each task at the end of the sequence. Based on clustering the Mid scale dataset 6DS into 4 semantic-split groups of facts. * assumes access to all the data in one learning phase  }
 \begin{tabular}{ | l | c| c | c | c | c | c |}
 \hline
 Method & $T_1$ &$T_2$&$T_3$ & $T_4$&avg & generalized\\  \hline
% %
 Finetuning& 11.7& 18.2 &24.4& 15.0&17.3 & - \\  \hline  	
 Int. Synapses~\cite{zenke2017improved}&  12.0& 18.2 & 0.246& 9.17&16.0 &- \\  \hline
 MAS~\cite{mas}& 13.9 &50.8 & 24.8&11.7&25.3 &-\\  \hline  
 Joint Training*& &  & & &  &- \\ \hline
% %{'res_b1': 0.29504979244916801, 'res_b2': 0.23784487176071828, 'res_b4': 0.39652403591452356, 'res_all': 0.28506532531130085, 'res_b3': 0.23933478694529423}		
 \end{tabular}

\vspace*{-0.2cm} 
 \end{table}
 
 
